Reinforcement Learning Improves LLM Accuracy and Reasoning in Disease Classification from Radiology Reports

Accurate disease classification from radiology reports is essential for many applications. While supervised fine-tuning (SFT) of lightweight LLMs improves accuracy, it can degrade reasoning. We propose a two-stage approach: SFT on disease labels followed by Group Relative Policy Optimization (GRPO) to refine predictions by optimizing accuracy and format without reasoning supervision. Across three radiologist-annotated datasets, SFT outperformed baselines and GRPO further improved classification and enhanced reasoning recall and comprehensiveness.

==> tables/stab_accuracy_per_disease.tex <==
\begin{tabular}{lccccccccc}
\toprule
Disease & \multicolumn{3}{c}{Micro precision} & \multicolumn{3}{c}{Micro recall} & \multicolumn{3}{c}{Micro F1} \\
\cmidrule(rl){2-4}\cmidrule(rl){5-7}\cmidrule(rl){8-10}
 & Baseline & SFT & \makecell[c]{SFT\\+GRPO} & Baseline & SFT & \makecell[c]{SFT\\+GRPO} & Baseline & SFT & \makecell[c]{SFT\\+GRPO} \\
\hline
\rowcolor{graybg} \multicolumn{10}{c}{Llama} \\
Atelectasis      & 0.333 & 0.690 & 0.750 & 0.040 & 0.800 & 0.960 & 0.071 & 0.741 & 0.842 \\
Cardiomegaly     & 1.000 & 1.000 & 1.000 & 0.086 & 0.971 & 0.914 & 0.158 & 0.985 & 0.955 \\
Consolidation    & -    & 0.400 & 0.400 & 0.000 & 1.000 & 1.000 & -    & 0.571 & 0.571 \\
Edema            & -    & 0.944 & 0.947 & 0.000 & 0.944 & 1.000 & -    & 0.944 & 0.973 \\
Fracture         & -    & 1.000 & 1.000 & 0.000 & 0.667 & 0.667 & -    & 0.800 & 0.800 \\
Lung opacity     & 1.000 & 0.824 & 0.882 & 0.030 & 0.424 & 0.455 & 0.058 & 0.560 & 0.600 \\
Pleural effusion & 0.750 & 0.935 & 0.938 & 0.581 & 0.935 & 0.968 & 0.655 & 0.935 & 0.953 \\
Pneumonia        & 0.600 & 1.000 & 0.600 & 0.600 & 0.200 & 0.600 & 0.600 & 0.333 & 0.600 \\
Pneumothorax     & -    & 0.667 & 1.000 & 0.000 & 0.667 & 1.000 & -    & 0.667 & 1.000 \\
Support devices  & -    & 1.000 & 0.905 & 0.000 & 0.438 & 0.594 & -    & 0.609 & 0.717 \\
\rowcolor{graybg} \multicolumn{10}{c}{Qwen} \\
Atelectasis      & 0.308 & 0.737 & 0.667 & 0.160 & 0.560 & 0.640 & 0.211 & 0.636 & 0.653 \\
Cardiomegaly     & 1.000 & 0.938 & 0.941 & 0.286 & 0.857 & 0.914 & 0.445 & 0.896 & 0.927 \\
Consolidation    & 0.333 & 0.500 & 0.500 & 0.500 & 0.500 & 0.500 & 0.400 & 0.500 & 0.500 \\
Edema            & 1.000 & 0.800 & 0.778 & 0.056 & 0.667 & 0.778 & 0.106 & 0.727 & 0.778 \\
Fracture         & -    & 1.000 & 0.750 & 0.000 & 0.667 & 0.500 & -    & 0.800 & 0.600 \\
Lung opacity     & 1.000 & 0.667 & 0.917 & 0.091 & 0.182 & 0.333 & 0.167 & 0.286 & 0.489 \\
Pleural effusion & 1.000 & 0.941 & 0.913 & 0.129 & 0.516 & 0.677 & 0.229 & 0.667 & 0.777 \\
Pneumonia        & 0.400 & 0.250 & 0.500 & 0.800 & 0.200 & 0.800 & 0.533 & 0.222 & 0.615 \\
Pneumothorax     & 0.333 & 1.000 & 1.000 & 0.333 & 0.333 & 1.000 & 0.333 & 0.500 & 1.000 \\
Support devices  & -    & 0.818 & 0.955 & 0.000 & 0.563 & 0.656 & -    & 0.667 & 0.778 \\
\rowcolor{graybg} \multicolumn{10}{c}{Phi4} \\
Atelectasis      & 0.640 & 0.636 & 0.667 & 0.640 & 0.560 & 0.800 & 0.640 & 0.596 & 0.727 \\
Cardiomegaly     & 1.000 & 1.000 & 0.958 & 0.657 & 0.486 & 0.657 & 0.793 & 0.654 & 0.779 \\
Consolidation    & 0.000 & 0.250 & 0.400 & 0.000 & 0.500 & 1.000 & -    & 0.333 & 0.571 \\
Edema            & -    & 0.923 & 0.789 & 0.000 & 0.667 & 0.833 & -    & 0.774 & 0.810 \\
Fracture         & -    & 1.000 & 0.714 & 0.000 & 0.833 & 0.833 & -    & 0.909 & 0.769 \\
Lung opacity     & -    & 1.000 & 0.833 & 0.000 & 0.182 & 0.303 & -    & 0.308 & 0.444 \\
Pleural effusion & 0.800 & 0.957 & 0.871 & 0.774 & 0.710 & 0.871 & 0.787 & 0.815 & 0.871 \\
Pneumonia        & 0.238 & 0.600 & 0.333 & 1.000 & 0.600 & 0.400 & 0.384 & 0.600 & 0.363 \\
Pneumothorax     & 0.750 & 1.000 & 1.000 & 1.000 & 0.333 & 0.333 & 0.857 & 0.500 & 0.500 \\
Support devices  & -    & 0.944 & 0.952 & 0.000 & 0.531 & 0.625 & -    & 0.680 & 0.755 \\
\hline
\end{tabular}


==> tables/stab_comparing.tex <==
\begin{tabular}{llcc}
\toprule
Dataset & Model & \makecell[c]{SFT disease\\ + GRPO} & \makecell[c]{SFT disease \\+ SFT reasoning} \\ 
\midrule
\rowcolor{graybg} \multicolumn{4}{c}{F1}\\ 
MIMIC & Qwen & 0.729 [0.665, 0.786] & 0.652 [0.564, 0.724] \\ 
~ & Llama & 0.826 [0.775, 0.871] & 0.805 [0.758, 0.848] \\ 
~ & Phi3 & 0.712 [0.651, 0.773] & 0.689 [0.626, 0.754] \\ 
\midrule
NIH-CXR & Qwen & 0.824 [0.752, 0.880] & 0.836 [0.780, 0.888] \\ 
~ & Llama & 0.862 [0.813, 0.903] & 0.895 [0.842, 0.908] \\ 
~ & Phi3 & 0.689 [0.617, 0.745] & 0.653 [0.592, 0.705] \\ 
\midrule
MIDRC & Qwen & 0.661 [0.562, 0.748] & 0.792 [0.738, 0.846] \\ 
~ & Llama & 0.967 [0.942, 0.987] & 0.873 [0.838, 0.903] \\ 
~ & Phi3 & 0.535 [0.396, 0.610] & 0.562 [0.415, 0.583] \\ 
\rowcolor{graybg} \multicolumn{4}{c}{Reasoning recall}\\ 
MIMIC & Qwen & 0.725 [0.660, 0.793] & 0.751 [0.676, 0.827] \\ 
~ & Llama & 0.647 [0.556, 0.739] & 0.763 [0.681, 0.836] \\ 
~ & Phi3 & 0.714 [0.644, 0.785] & 0.746 [0.679, 0.812] \\
\midrule
NIH-CXR & Qwen & 0.792 [0.713, 0.870] & 0.833 [0.725, 0.924] \\ 
~ & Llama & 0.567 [0.430, 0.702] & 0.650 [0.512, 0.779] \\ 
~ & Phi3 & 0.692 [0.606, 0.773] & 0.754 [0.672, 0.835] \\ 
\midrule
MIDRC & Qwen & 0.664 [0.559, 0.750] & 0.792 [0.738, 0.846] \\ 
~ & Llama & 0.798 [0.685, 0.894] & 0.871 [0.838, 0.903] \\ 
~ & Phi3 & 0.588 [0.479, 0.700] & 0.538 [0.415, 0.583] \\ 
\rowcolor{graybg} \multicolumn{4}{c}{Reasoning comprehensiveness}\\ 
MIMIC & Qwen & 0.922 [0.868, 0.969] & 0.825 [0.756, 0.887] \\ 
~ & Llama & 0.743 [0.639, 0.839] & 0.786 [0.697, 0.857] \\ 
~ & Phi3 & 0.942 [0.892, 0.980] & 0.946 [0.898, 0.984] \\ 
\midrule
NIH-CXR & Qwen & 0.916 [0.846, 0.972] & 0.934 [0.859, 0.983] \\ 
~ & Llama & 0.576 [0.425, 0.727] & 0.667 [0.508, 0.806] \\ 
~ & Phi3 & 0.976 [0.943, 1.000] & 0.976 [0.934, 1.000] \\ 
\midrule
MIDRC & Qwen & 0.933 [0.888, 0.977] & 0.948 [0.910, 0.983] \\ 
~ & Llama & 0.805 [0.696, 0.903] & 0.640 [0.493, 0.766] \\ 
~ & Phi3 & 0.847 [0.747, 0.926] & 0.636 [0.500, 0.753] \\ 
\bottomrule
\end{tabular}

==> tables/stab_distribution.tex <==
\begin{tabular}{lrrrrrr}
\toprule
& \multicolumn{3}{c}{MIMIC-CXR}\\
\cmidrule{2-4}
Disease & Training & Reasoning & Evaluation & NIH-CXR & MIRDC & Evaluation-Silver \\ 
\midrule
Atelectasis & 0.203 & 0.230 & 0.27 & 0.12 & 0.00 & 0.217\\ 
Cardiomegaly & 0.176 & 0.215 & 0.35 & 0.01 & 0.06&0.198 \\ 
Consolidation & 0.035 & 0.015 & 0.02 & 0.04 & 0.02&0.033 \\ 
Edema & 0.084 & 0.090 & 0.18 & 0.06 & 0.00&0.088 \\ 
Enlarged cardiomediastinum & 0.011 & 0.010 & 0.01 & 0.00 & 0.00&0.010 \\ 
Fracture & 0.031 & 0.040 & 0.06 & 0.02 & 0.00&0.027 \\ 
Lung lesion & 0.009 & 0.005 & 0.00 & 0.02 & 0.00&0.011 \\ 
Lung opacity & 0.173 & 0.150 & 0.33 & 0.76 & 0.98&0.196 \\ 
Pleural effusion & 0.201 & 0.215 & 0.31 & 0.62 & 0.78 &0.205 \\ 
Pleural other & 0.006 & 0.010 & 0.00 & 0.00 & 0.00&0.003 \\ 
Pneumonia & 0.033 & 0.020 & 0.05 & 0.02 & 0.02&0.028 \\ 
Pneumothorax & 0.025 & 0.040 & 0.03 & 0.10 & 0.02 &0.025\\ 
Support devices & 0.200 & 0.205 & 0.25 & 0.68 & 0.70 & 0.212 \\ 
\bottomrule
\end{tabular}

==> tables/stab_mimic_before_ensemble.tex <==

\begin{tabular}{l lc c c c cc c c c c}
\toprule
 &  & \multicolumn{5}{c}{Precision} & \multicolumn{5}{c}{Recall} \\
\cmidrule(rl){3-7}\cmidrule(rl){8-12}
Model & Method &  1 & 2 & 3 & 4 & 5 & 1 & 2 & 3 & 4 & 5 \\
\midrule
Llama & Baseline   & 0.045 & 0.327 & 0.318 & 0.215 & 0.353 & 0.041 & 0.171 & 0.394 & 0.218 & 0.218 \\
      & SFT        & 0.828 & 0.796 & 0.808 & 0.829 & 0.801 & 0.699 & 0.689 & 0.699 & 0.705 & 0.710 \\
      & SFT+GRPO   & 0.721 & 0.723 & 0.766 & 0.779 & 0.785 & 0.736 & 0.731 & 0.731 & 0.694 & 0.736 \\
\midrule
Qwen  & Baseline   & 0.347 & 0.452 & 0.390 & 0.371 & 0.178 & 0.218 & 0.098 & 0.202 & 0.187 & 0.124 \\
      & SFT        & 0.787 & 0.819 & 0.803 & 0.806 & 0.828 & 0.554 & 0.539 & 0.570 & 0.539 & 0.523 \\
      & SFT+GRPO   & 0.800 & 0.791 & 0.828 & 0.776 & 0.799 & 0.601 & 0.648 & 0.648 & 0.627 & 0.596 \\
\midrule
Phi4  & Baseline   & 0.333 & 0.353 & 0.400 & 0.372 & 0.453 & 0.244 & 0.378 & 0.383 & 0.378 & 0.399 \\
      & SFT        & 0.695 & 0.674 & 0.669 & 0.667 & 0.642 & 0.591 & 0.482 & 0.482 & 0.477 & 0.456 \\
      & SFT+GRPO   & 0.730 & 0.784 & 0.711 & 0.736 & 0.781 & 0.658 & 0.658 & 0.637 & 0.663 & 0.627 \\
\midrule
 & & \multicolumn{5}{c}{F1} & \multicolumn{3}{c}{Average} \\
 \cmidrule(rl){3-7}\cmidrule(rl){8-10}
 &  & 1 & 2 & 3 & 4 & 5 & Precision & Recall & F1 \\
\cmidrule(rl){1-10}
Llama & Baseline   & 0.043 & 0.225 & 0.352 & 0.216 & 0.270 & 0.251 & 0.208 & 0.228 \\
      & SFT        & 0.758 & 0.739 & 0.750 & 0.762 & 0.753 & 0.812 & 0.700 & 0.752 \\
      & SFT+GRPO   & 0.728 & 0.727 & 0.748 & 0.734 & 0.760 & 0.754 & 0.725 & 0.740 \\
\cmidrule(rl){1-10}
Qwen  & Baseline   & 0.268 & 0.161 & 0.266 & 0.249 & 0.146 & 0.347 & 0.165 & 0.218 \\
      & SFT        & 0.650 & 0.650 & 0.667 & 0.646 & 0.641 & 0.808 & 0.545 & 0.651 \\
      & SFT+GRPO   & 0.686 & 0.712 & 0.727 & 0.694 & 0.683 & 0.798 & 0.624 & 0.700 \\
\cmidrule(rl){1-10}
Phi4  & Baseline   & 0.282 & 0.365 & 0.391 & 0.375 & 0.424 & 0.382 & 0.356 & 0.367 \\
      & SFT        & 0.639 & 0.562 & 0.560 & 0.556 & 0.533 & 0.669 & 0.497 & 0.570 \\
      & SFT+GRPO   & 0.692 & 0.715 & 0.672 & 0.698 & 0.696 & 0.748 & 0.648 & 0.695 \\
\bottomrule
\end{tabular}



==> tables/stab_nih_before_ensemble.tex <==
\begin{tabular}{l lc c c c cc c c c c}
\toprule
 &  & \multicolumn{5}{c}{Precision} & \multicolumn{5}{c}{Recall} \\
\cmidrule(rl){3-7}\cmidrule(rl){8-12}
Model &  Method & 1 & 2 & 3 & 4 & 5 & 1 & 2 & 3 & 4 & 5 \\
\midrule
Llama & Baseline   & 0.206 & 0.319 & 0.269 & 0.246 & 0.286 & 0.108 & 0.186 & 0.137 & 0.137 & 0.176 \\
      & SFT        & 0.946 & 0.952 & 0.958 & 0.948 & 0.953 & 0.779 & 0.784 & 0.784 & 0.799 & 0.794 \\
      & SFT+GRPO   & 0.900 & 0.911 & 0.897 & 0.900 & 0.922 & 0.922 & 0.907 & 0.936 & 0.931 & 0.926 \\
\midrule
Qwen  & Baseline   & 0.365 & 0.186 & 0.293 & 0.327 & 0.228 & 0.225 & 0.108 & 0.167 & 0.176 & 0.127 \\
      & SFT        & 0.817 & 0.845 & 0.842 & 0.834 & 0.857 & 0.613 & 0.642 & 0.627 & 0.618 & 0.647 \\
      & SFT+GRPO   & 0.739 & 0.795 & 0.781 & 0.771 & 0.770 & 0.569 & 0.686 & 0.647 & 0.642 & 0.672 \\
\midrule
Phi4  & Baseline   & 0.321 & 0.346 & 0.307 & 0.346 & 0.345 & 0.245 & 0.275 & 0.225 & 0.275 & 0.279 \\
      & SFT        & 0.753 & 0.709 & 0.637 & 0.725 & 0.647 & 0.539 & 0.525 & 0.456 & 0.569 & 0.475 \\
      & SFT+GRPO   & 0.765 & 0.740 & 0.739 & 0.743 & 0.675 & 0.608 & 0.544 & 0.583 & 0.623 & 0.510 \\
\midrule
 & & \multicolumn{5}{c}{F1} & \multicolumn{3}{c}{Average} \\
 \cmidrule(rl){3-7}\cmidrule(rl){8-10}
 &  & 1 & 2 & 3 & 4 & 5 & Precision & Recall & F1 \\
\cmidrule(rl){1-10}
Llama & Baseline   & 0.142 & 0.235 & 0.182 & 0.176 & 0.218 & 0.265 & 0.149 & 0.191 \\
      & SFT        & 0.854 & 0.860 & 0.862 & 0.867 & 0.866 & 0.951 & 0.788 & 0.862 \\
      & SFT+GRPO   & 0.911 & 0.909 & 0.916 & 0.915 & 0.924 & 0.906 & 0.924 & 0.915 \\
\cmidrule(rl){1-10}
Qwen  & Baseline   & 0.278 & 0.137 & 0.213 & 0.229 & 0.163 & 0.280 & 0.161 & 0.204 \\
      & SFT        & 0.700 & 0.730 & 0.719 & 0.710 & 0.737 & 0.839 & 0.629 & 0.719 \\
      & SFT+GRPO   & 0.643 & 0.736 & 0.708 & 0.701 & 0.718 & 0.771 & 0.643 & 0.701 \\
\cmidrule(rl){1-10}
Phi4  & Baseline   & 0.278 & 0.306 & 0.260 & 0.306 & 0.309 & 0.333 & 0.260 & 0.292 \\
      & SFT        & 0.628 & 0.603 & 0.532 & 0.638 & 0.548 & 0.694 & 0.513 & 0.590 \\
      & SFT+GRPO   & 0.678 & 0.627 & 0.652 & 0.678 & 0.581 & 0.732 & 0.574 & 0.643 \\
\bottomrule
\end{tabular}


==> tables/stab_reasoning.tex <==
\begin{tabular}{llccc}
\toprule
Dataset & Model & Baseline & SFT & SFT + GRPO \\
\midrule
\rowcolor{graybg} \multicolumn{5}{c}{Reasoning recall} \\ 
MIMIC & Qwen & 0.435 [0.357, 0.513] & 0.456 [0.376, 0.541] & 0.725 [0.660, 0.793] \\ 
~ & Llama & 0.171 [0.099, 0.246] & 0.000 [0.000, 0.000] & 0.647 [0.556, 0.739] \\ 
~ & Phi3 & 0.400 [0.330, 0.466] & 0.715 [0.660, 0.773] & 0.714 [0.644, 0.785] \\ 
\midrule
NIH-CXR & Qwen & 0.462 [0.362, 0.573] & 0.650 [0.518, 0.779] & 0.792 [0.713, 0.870] \\ 
~ & Llama & 0.208 [0.131, 0.288] & 0.000 [0.000, 0.000] & 0.567 [0.430, 0.702] \\ 
~ & Phi3 & 0.525 [0.446, 0.603] & 0.625 [0.508, 0.735] & 0.692 [0.606, 0.773] \\ 
\midrule
MIDRC & Qwen & 0.362 [0.290, 0.437] & 0.529 [0.419, 0.636] & 0.664 [0.559, 0.750] \\ 
~ & Llama & 0.277 [0.171, 0.378] & 0.000 [0.000, 0.000] & 0.798 [0.685, 0.894] \\ 
~ & Phi3 & 0.378 [0.285, 0.487] & 0.496 [0.387, 0.607] & 0.588 [0.479, 0.700] \\ 
\rowcolor{graybg} \multicolumn{5}{c}{Reasoning comprehensiveness} \\ 
MIMIC & Qwen & 0.742 [0.635, 0.841] & 0.661 [0.537, 0.787] & 0.922 [0.868, 0.969] \\ 
~ & Llama & 0.421 [0.270, 0.571] & 0.000 [0.000, 0.000] & 0.743 [0.639, 0.839] \\ 
~ & Phi3 & 0.606 [0.508, 0.704] & 0.957 [0.918, 0.990] & 0.942 [0.892, 0.980] \\ 
\midrule
NIH-CXR & Qwen & 0.724 [0.583, 0.862] & 0.790 [0.649, 0.912] & 0.916 [0.846, 0.972] \\ 
~ & Llama & 0.339 [0.186, 0.500] & 0.000 [0.000, 0.000] & 0.576 [0.425, 0.727] \\ 
~ & Phi3 & 0.768 [0.652, 0.867] & 0.933 [0.855, 0.988] & 0.976 [0.943, 1.000] \\
\midrule
MIDRC & Qwen & 0.839 [0.721, 0.959] & 0.778 [0.659, 0.877] & 0.933 [0.888, 0.977] \\ 
~ & Llama & 0.403 [0.273, 0.532] & 0.000 [0.000, 0.000] & 0.805 [0.696, 0.903] \\ 
~ & Phi3 & 0.838 [0.750, 0.915] & 0.780 [0.678, 0.864] & 0.847 [0.747, 0.926] \\ 
\bottomrule
\end{tabular}

==> tables/stab_silver_data.tex <==
\begin{tabular}{lccccccccc}
\toprule
\multirow{2}{*}{Model} & \multicolumn{3}{c}{Micro precision} & \multicolumn{3}{c}{Micro recall} & \multicolumn{3}{c}{Micro F1} \\
\cmidrule(rl){2-4}\cmidrule(rl){5-7}\cmidrule(rl){8-10}
 & Baseline & SFT & \makecell[c]{SFT\\+GRPO} & Baseline & SFT & \makecell[c]{SFT\\+GRPO} & Baseline & SFT & \makecell[c]{SFT\\+GRPO} \\
\midrule
Qwen  & 0.489 & \textbf{0.787} & 0.778 & 0.389 & 0.539 & \textbf{0.648} & 0.433 & 0.640 & \textbf{0.707} \\
Llama & 0.454 & \textbf{0.775} & 0.771 & 0.436 & \textbf{0.847} & 0.839 & 0.445 & \textbf{0.809} & 0.804 \\
Phi3  & 0.405 & 0.683 & \textbf{0.708} & 0.414 & 0.548 & \textbf{0.615} & 0.409 & 0.608 & \textbf{0.658} \\
\bottomrule
\end{tabular}



==> tables/stab_variants.tex <==
\begin{tabular}{llccc}
\toprule
Dataset & Model & Baseline & SFT & SFT + GRPO \\
\midrule
\rowcolor{graybg} \multicolumn{5}{c}{Micro precision} \\ 
MIMIC & Qwen & 0.452 [0.311, 0.586] & 0.811 [0.744, 0.871] & 0.824 [0.764, 0.881] \\ 
~ & Llama & 0.684 [0.528, 0.824] & 0.873 [0.825, 0.919] & 0.882 [0.831, 0.931] \\ 
~ & Phi3 & 0.511 [0.431, 0.588] & 0.845 [0.776, 0.908] & 0.791 [0.731, 0.849] \\ 
~ & GPT4-o & 0.758 & - & - \\ 
\midrule
NIH-CXR & Qwen & 0.362 [0.255, 0.462] & 0.907 [0.846, 0.960] & 0.875 [0.804, 0.940] \\ 
~ & Llama & 0.286 [0.160, 0.412] & 0.929 [0.856, 0.988] & 0.870 [0.805, 0.929] \\ 
~ & Phi3 & 0.429 [0.341, 0.519] & 0.795 [0.705, 0.885] & 0.829 [0.747, 0.902] \\ 
~ & GPT4-o & 0.776 & - & - \\ 
\midrule
MIDRC & Qwen & 0.298 [0.164, 0.427] & 0.827 [0.738, 0.908] & 0.767 [0.674, 0.845] \\ 
~ & Llama & 0.254 [0.167, 0.329] & 0.980 [0.949, 1.000] & 0.951 [0.911, 0.991] \\ 
~ & Phi3 & 0.243 [0.149, 0.329] & 0.582 [0.439, 0.646] & 0.560 [0.494, 0.714] \\  
~ & GPT4-o & 0.667 & - & - \\ 
\rowcolor{graybg} \multicolumn{5}{c}{Micro recall}\\ 
MIMIC & Qwen & 0.145 [0.091, 0.208] & 0.534 [0.449, 0.610] & 0.653 [0.586, 0.722] \\ 
~ & Llama & 0.135 [0.088, 0.185] & 0.710 [0.646, 0.771] & 0.777 [0.718, 0.839] \\ 
~ & Phi3 & 0.368 [0.304, 0.436] & 0.508 [0.429, 0.582] & 0.648 [0.571, 0.720] \\ 
~ & GPT4-o & 0.907 & - & ~ \\ 
\midrule
NIH-CXR & Qwen & 0.179 [0.121, 0.250] & 0.752 [0.677, 0.823] & 0.778 [0.701, 0.850] \\ 
~ & Llama & 0.137 [0.075, 0.218] & 0.778 [0.717, 0.848] & 0.855 [0.789, 0.917] \\ 
~ & Phi3 & 0.359 [0.282, 0.432] & 0.496 [0.407, 0.586] & 0.590 [0.500, 0.661] \\ 
~ & GPT4-o & 0.949 & - & ~ \\ 
\midrule
MIDRC & Qwen & 0.143 [0.071, 0.218] & 0.563 [0.480, 0.639] & 0.580 [0.587, 0.675] \\ 
~ & Llama & 0.143 [0.086, 0.208] & 0.824 [0.772, 0.878] & 0.983 [0.957, 1.000] \\ 
~ & Phi3 & 0.151 [0.090, 0.218] & 0.487 [0.275, 0.488] & 0.513 [0.328, 0.541] \\ 
~ & GPT4-o & 0.984 & - & - \\ 
\rowcolor{graybg} \multicolumn{5}{c}{Micro F1}\\ 
MIMIC & Qwen & 0.220 [0.139, 0.296] & 0.644 [0.574, 0.710] & 0.729 [0.665, 0.786] \\ 
~ & Llama & 0.225 [0.157, 0.299] & 0.783 [0.732, 0.833] & 0.826 [0.775, 0.871] \\ 
~ & Phi3 & 0.428 [0.359, 0.494] & 0.635 [0.566, 0.702] & 0.712 [0.651, 0.773] \\ 
~ & GPT4-o & 0.826 & - & - \\ 
\midrule
NIH-CXR & Qwen & 0.240 [0.167, 0.320] & 0.822 [0.763, 0.872] & 0.824 [0.752, 0.880] \\ 
~ & Llama & 0.185 [0.098, 0.276] & 0.847 [0.796, 0.900] & 0.862 [0.813, 0.903] \\ 
~ & Phi3 & 0.391 [0.307, 0.467] & 0.611 [0.523, 0.694] & 0.689 [0.617, 0.745] \\ 
~ & GPT4-o & 0.854 & - & - \\ 
\midrule
MIDRC & Qwen & 0.193 [0.096, 0.295] & 0.670 [0.586, 0.745] & 0.661 [0.562, 0.748] \\ 
~ & Llama & 0.183 [0.112, 0.254] & 0.895 [0.863, 0.926] & 0.967 [0.942, 0.987] \\ 
~ & Phi3 & 0.186 [0.111, 0.263] & 0.509 [0.346, 0.545] & 0.535 [0.396, 0.610] \\ 
~ & GPT4-o & 0.795 & - & - \\ 
\bottomrule
\end{tabular}

==> tables/tab_statistics.tex <==
\begin{tabular}{lcccccc}
\toprule
& \multicolumn{4}{c}{MIMIC-CXR}\\
\cmidrule{2-5}
Disease & Training & Reasoning & Evaluation & \makecell[c]{Eval-Silver} & NIH-CXR & MIRDC \\ 
\midrule
Usage & \makecell[c]{Fine-tuning \\\& GRPO training} & \makecell[c]{Fine-tuning \\(reasoning)} & Evaluation & Evaluation & Evaluation & Evaluation \\ 
Annotator & GPT4-o & GPT4-o & Radiologists & GPT4-o & Radiologists & Radiologists \\ 
Reports & 2,000 & 200 & 100 & 1,000 & 50 & 50 \\ 
Average length & 47.9 & 45.8 & 60 & 48.1 & 52 & 58.3 \\ 
Average labels & 1.59 & 1.65 & 1.93 & 1.61 & 2.52 & 2.59 \\ 
Disease & ~ & ~ & ~ & ~ & ~ & ~ \\ 
~~~~Atelectasis & 0.203 & 0.230 & 0.270 & 0.217 & 0.120 & 0.000 \\ 
~~~~Cardiomegaly & 0.176 & 0.215 & 0.350 & 0.198 & 0.010 & 0.060 \\ 
~~~~Consolidation & 0.035 & 0.015 & 0.020 & 0.033 & 0.040 & 0.020 \\ 
~~~~Edema & 0.084 & 0.090 & 0.180 & 0.088 & 0.060 & 0.000 \\ 
~~~~Enlarged card. & 0.011 & 0.010 & 0.010 & 0.010 & 0.000 & 0.000 \\ 
~~~~Fracture & 0.031 & 0.040 & 0.060 & 0.027 & 0.020 & 0.000 \\ 
~~~~Lung lesion & 0.009 & 0.005 & 0.000 & 0.011 & 0.020 & 0.000 \\ 
~~~~Lung opacity & 0.173 & 0.150 & 0.330 & 0.196 & 0.760 & 0.980 \\ 
~~~~Pleural effusion & 0.201 & 0.215 & 0.310 & 0.205 & 0.620 & 0.780 \\ 
~~~~Pleural other & 0.006 & 0.010 & 0.000 & 0.003 & 0.000 & 0.000 \\ 
~~~~Pneumonia & 0.033 & 0.020 & 0.050 & 0.028 & 0.020 & 0.020 \\ 
~~~~Pneumothorax & 0.025 & 0.040 & 0.030 & 0.025 & 0.100 & 0.020 \\ 
~~~~Support devices & 0.200 & 0.205 & 0.250 & 0.212 & 0.680 & 0.700 \\ 
\bottomrule
\multicolumn{7}{l}{card. - cardiomediastinum.}\\
\end{tabular}

==> tables/tab_statistics_v0.tex <==
\begin{tabular}{lllrrr}
\toprule
Dataset & Usage & Annotator & Reports & \makecell[r]{Average\\length} & \makecell[r]{Average\\labels} \\
\midrule
MIMIC-CXR\\
~~Training & Fine-tuning \& GRPO training & GPT4-o & 2,000 & 47.9 & 1.59 \\ 
~~Teasoning & Fine-tuning (reasoning) & GPT4-o & 200 & 45.8 & 1.65 \\ 
~~Evaluation & Evaluation & Radiologists & 100 & 60.0 & 1.93 \\ 
~~Evaluation-Silver & Evaluation & GPT4-o & 1,000 & 48.1 & 1.61 \\ 
NIH-CXR & Evaluation & Radiologists & 50 & 52.0 & 2.52 \\ 
MIRDC & Evaluation & Radiologists & 50 & 58.3 & 2.59 \\ 
\bottomrule
\end{tabular}

==> tables_revision/stab_distribution.tex <==
\begin{tabular}{lrrrrrr}
\toprule
& \multicolumn{3}{c}{MIMIC-CXR}\\
\cmidrule{2-4}
Disease & Training & Reasoning & Evaluation & NIH-CXR & MIRDC & Evaluation-Silver \\ 
\midrule
Atelectasis & 0.203 & 0.230 & 0.27 & 0.12 & 0.00 & 0.217\\ 
Cardiomegaly & 0.176 & 0.215 & 0.35 & 0.01 & 0.06&0.198 \\ 
Consolidation & 0.035 & 0.015 & 0.02 & 0.04 & 0.02&0.033 \\ 
Edema & 0.084 & 0.090 & 0.18 & 0.06 & 0.00&0.088 \\ 
Enlarged cardiomediastinum & 0.011 & 0.010 & 0.01 & 0.00 & 0.00&0.010 \\ 
Fracture & 0.031 & 0.040 & 0.06 & 0.02 & 0.00&0.027 \\ 
Lung lesion & 0.009 & 0.005 & 0.00 & 0.02 & 0.00&0.011 \\ 
Lung opacity & 0.173 & 0.150 & 0.33 & 0.76 & 0.98&0.196 \\ 
Pleural effusion & 0.201 & 0.215 & 0.31 & 0.62 & 0.78 &0.205 \\ 
Pleural other & 0.006 & 0.010 & 0.00 & 0.00 & 0.00&0.003 \\ 
Pneumonia & 0.033 & 0.020 & 0.05 & 0.02 & 0.02&0.028 \\ 
Pneumothorax & 0.025 & 0.040 & 0.03 & 0.10 & 0.02 &0.025\\ 
Support devices & 0.200 & 0.205 & 0.25 & 0.68 & 0.70 & 0.212 \\ 
\bottomrule
\end{tabular}

==> tables_revision/stab_nih_before_ensemble.tex <==
\begin{tabular}{l lc c c c cc c c c c}
\toprule
 &  & \multicolumn{5}{c}{Precision} & \multicolumn{5}{c}{Recall} \\
\cmidrule(rl){3-7}\cmidrule(rl){8-12}
Model &  Method & 1 & 2 & 3 & 4 & 5 & 1 & 2 & 3 & 4 & 5 \\
\midrule
Llama & Baseline   & 0.206 & 0.319 & 0.269 & 0.246 & 0.286 & 0.108 & 0.186 & 0.137 & 0.137 & 0.176 \\
      & SFT        & 0.946 & 0.952 & 0.958 & 0.948 & 0.953 & 0.779 & 0.784 & 0.784 & 0.799 & 0.794 \\
      & SFT+GRPO   & 0.900 & 0.911 & 0.897 & 0.900 & 0.922 & 0.922 & 0.907 & 0.936 & 0.931 & 0.926 \\
\midrule
Qwen  & Baseline   & 0.365 & 0.186 & 0.293 & 0.327 & 0.228 & 0.225 & 0.108 & 0.167 & 0.176 & 0.127 \\
      & SFT        & 0.817 & 0.845 & 0.842 & 0.834 & 0.857 & 0.613 & 0.642 & 0.627 & 0.618 & 0.647 \\
      & SFT+GRPO   & 0.739 & 0.795 & 0.781 & 0.771 & 0.770 & 0.569 & 0.686 & 0.647 & 0.642 & 0.672 \\
\midrule
Phi4  & Baseline   & 0.321 & 0.346 & 0.307 & 0.346 & 0.345 & 0.245 & 0.275 & 0.225 & 0.275 & 0.279 \\
      & SFT        & 0.753 & 0.709 & 0.637 & 0.725 & 0.647 & 0.539 & 0.525 & 0.456 & 0.569 & 0.475 \\
      & SFT+GRPO   & 0.765 & 0.740 & 0.739 & 0.743 & 0.675 & 0.608 & 0.544 & 0.583 & 0.623 & 0.510 \\
\midrule
 & & \multicolumn{5}{c}{F1} & \multicolumn{3}{c}{Average} \\
 \cmidrule(rl){3-7}\cmidrule(rl){8-10}
 &  & 1 & 2 & 3 & 4 & 5 & Precision & Recall & F1 \\
\cmidrule(rl){1-10}
Llama & Baseline   & 0.142 & 0.235 & 0.182 & 0.176 & 0.218 & 0.265 & 0.149 & 0.191 \\
      & SFT        & 0.854 & 0.860 & 0.862 & 0.867 & 0.866 & 0.951 & 0.788 & 0.862 \\
      & SFT+GRPO   & 0.911 & 0.909 & 0.916 & 0.915 & 0.924 & 0.906 & 0.924 & 0.915 \\
\cmidrule(rl){1-10}
Qwen  & Baseline   & 0.278 & 0.137 & 0.213 & 0.229 & 0.163 & 0.280 & 0.161 & 0.204 \\
      & SFT        & 0.700 & 0.730 & 0.719 & 0.710 & 0.737 & 0.839 & 0.629 & 0.719 \\
      & SFT+GRPO   & 0.643 & 0.736 & 0.708 & 0.701 & 0.718 & 0.771 & 0.643 & 0.701 \\
\cmidrule(rl){1-10}
Phi4  & Baseline   & 0.278 & 0.306 & 0.260 & 0.306 & 0.309 & 0.333 & 0.260 & 0.292 \\
      & SFT        & 0.628 & 0.603 & 0.532 & 0.638 & 0.548 & 0.694 & 0.513 & 0.590 \\
      & SFT+GRPO   & 0.678 & 0.627 & 0.652 & 0.678 & 0.581 & 0.732 & 0.574 & 0.643 \\
\bottomrule
\end{tabular}


==> tables_revision/stab_reasoning2.tex <==
\begin{tblr}{
    colspec={lll@{~}ll@{~}ll@{~}l},
    hline{1,3,Z}= {.5pt,solid},
}
& & \SetCell[c=2]{l}{Baseline} & & \SetCell[c=2]{l}{SFT} && \SetCell[c=2]{l}{SFT + GRPO} & \\
\cline[r]{3-4}\cline[r]{5-6}\cline{7-8}
 & & & [95\% CI] && [95\% CI] && [95\% CI]\\
\SetCell[c=5]{l}{\textbf{Reasoning recall}} \\ 
\hline[gray8]
\SetCell[c=2]{l}{MIMIC} \\
\cline[gray9]{2-8}
& Qwen-3B & 0.435 &[0.357, 0.513] & 0.456 &[0.376, 0.541] & 0.725 &[0.660, 0.793] \\ 
\cline[gray8]{2-8}
~ & Llama & 0.171 &[0.099, 0.246] & 0.000 &[0.000, 0.000] & 0.647 &[0.556, 0.739] \\ 
\cline[gray8]{2-8}
~ & Phi3 & 0.400 &[0.330, 0.466] & 0.715 &[0.660, 0.773] & 0.714 &[0.644, 0.785] \\ 
\hline[gray8]
\SetCell[c=2]{l}{NIH-CXR} \\
\cline[gray9]{2-8}
& Qwen-3B & 0.462 &[0.362, 0.573] & 0.650 &[0.518, 0.779] & 0.792 &[0.713, 0.870] \\ 
\cline[gray9]{2-8}
~ & Llama & 0.208 &[0.131, 0.288] & 0.000 &[0.000, 0.000] & 0.567 &[0.430, 0.702] \\ 
\cline[gray9]{2-8}
~ & Phi3 & 0.525 &[0.446, 0.603] & 0.625 &[0.508, 0.735] & 0.692 &[0.606, 0.773] \\ 
\hline[gray8]
\SetCell[c=2]{l}{MIDRC} \\
\cline[gray9]{2-8}
& Qwen-3B & 0.362 &[0.290, 0.437] & 0.529 &[0.419, 0.636] & 0.664 &[0.559, 0.750] \\ 
\cline[gray9]{2-8}
~ & Llama & 0.277 &[0.171, 0.378] & 0.000 &[0.000, 0.000] & 0.798 &[0.685, 0.894] \\ 
\cline[gray9]{2-8}
~ & Phi3 & 0.378 &[0.285, 0.487] & 0.496 &[0.387, 0.607] & 0.588 &[0.479, 0.700] \\ 
\hline[gray8]
\SetCell[c=5]{l}{\textbf{Reasoning comprehensiveness}} \\ 
\hline[gray8]
\SetCell[c=2]{l}{MIMIC} \\
\cline[gray9]{2-8}
& Qwen-3B & 0.742 &[0.635, 0.841] & 0.661 &[0.537, 0.787] & 0.922 &[0.868, 0.969] \\ 
\cline[gray9]{2-8}
~ & Llama & 0.421 &[0.270, 0.571] & 0.000 &[0.000, 0.000] & 0.743 &[0.639, 0.839] \\ 
\cline[gray9]{2-8}
~ & Phi3 & 0.606 &[0.508, 0.704] & 0.957 &[0.918, 0.990] & 0.942 &[0.892, 0.980] \\ 
\hline[gray8]
\SetCell[c=2]{l}{NIH-CXR} \\
\cline[gray9]{2-8}
& Qwen-3B & 0.724 &[0.583, 0.862] & 0.790 &[0.649, 0.912] & 0.916 &[0.846, 0.972] \\ 
\cline[gray9]{2-8}
~ & Llama & 0.339 &[0.186, 0.500] & 0.000 &[0.000, 0.000] & 0.576 &[0.425, 0.727] \\ 
\cline[gray9]{2-8}
~ & Phi3 & 0.768 &[0.652, 0.867] & 0.933 &[0.855, 0.988] & 0.976 &[0.943, 1.000] \\
\hline[gray8]
\SetCell[c=2]{l}{MIDRC} \\
\cline[gray9]{2-8}
& Qwen-3B & 0.839 &[0.721, 0.959] & 0.778 &[0.659, 0.877] & 0.933 &[0.888, 0.977] \\ 
\cline[gray9]{2-8}
~ & Llama & 0.403 &[0.273, 0.532] & 0.000 &[0.000, 0.000] & 0.805 &[0.696, 0.903] \\ 
\cline[gray9]{2-8}
~ & Phi3 & 0.838 &[0.750, 0.915] & 0.780 &[0.678, 0.864] & 0.847 &[0.747, 0.926] \\ 
% \bottomrule
\end{tblr}

==> tables_revision/tab_statistics_v0.tex <==
\begin{tabular}{lllrrr}
\toprule
Dataset & Usage & Annotator & Reports & \makecell[r]{Average\\length} & \makecell[r]{Average\\labels} \\
\midrule
MIMIC-CXR\\
~~Training & Fine-tuning \& GRPO training & GPT4-o & 2,000 & 47.9 & 1.59 \\ 
~~Teasoning & Fine-tuning (reasoning) & GPT4-o & 200 & 45.8 & 1.65 \\ 
~~Evaluation & Evaluation & Radiologists & 100 & 60.0 & 1.93 \\ 
~~Evaluation-Silver & Evaluation & GPT4-o & 1,000 & 48.1 & 1.61 \\ 
NIH-CXR & Evaluation & Radiologists & 50 & 52.0 & 2.52 \\ 
MIRDC & Evaluation & Radiologists & 50 & 58.3 & 2.59 \\ 
\bottomrule
\end{tabular}
